Restricted orientation "liquid crystal" in two dimensions: Isotropic-nematic transition or liquid-gas (?)

We present Monte Carlo simulation results of the two-dimensional Zwanzig fluid, which consists of hard line segments which may orient either horizontally or vertically. At a certain critical fugacity, we observe a phase transition with a two-dimensional Ising critical point. Above the transition point, the system is in an ordered state, with the majority of particles being either horizontally or vertically aligned. In contrast to previous work, we identify the transition as being of the liquid-gas type, as opposed to isotropic-to-nematic. This interpretation naturally accounts for the observed Ising critical behavior. Furthermore, when the Zwanzig fluid is extended to more allowed particle orientations, we argue that in some cases the symmetry of a q-state Potts model with q>2 arises. This observation is used to interpret a number of previous results.

==> Makefile <==
NAME = fischer_vink_revised

fast:
	latex $(NAME)

dvi:
	make clean
	latex $(NAME)
	latex $(NAME)
	latex $(NAME)

ps:
	make clean
	make dvi
	dvips $(NAME).dvi $(NAME).ps

pdf:	
	make clean
	make dvi
	dvipdf $(NAME)

bib:
	make clean
	latex $(NAME)
	latex $(NAME)
	latex $(NAME)
	bibtex $(NAME)

tar:
	tar cvfz $(NAME).tgz $(NAME).tex *.eps *.bbl Makefile

submit:
	tar cvfz submit.tgz $(NAME).tex *.eps *.bbl

view:
	xdvi -s 4 $(NAME)&

clean:
	rm -f *.aux *.log *.blg *.toc *.out *.fgx *.tbx *.lof *.lot \
              *.dvi *.idx *.ilg *.ind $(NAME).ps *.pdf *.end \
             cites.XXX submit.tgz $(NAME).tgz

veryclean:
	make clean
	rm -f *.bbl

pdffigs: $(patsubst %.eps,%.pdf,$(wildcard *.eps))

%.pdf : %.eps
	epstopdf $<

spell:
	aspell --mode=tex -c $(NAME).tex


